Single-pulse analysis and average emission characteristics of PSR J1820-0427 from observations made with the MWA and uGMRT

We have studied the pulse-to-pulse variability in PSR J1820--0427 and its frequency dependence using high-quality, wide-band observations made from the upgraded Giant Metrewave Radio Telescope (uGMRT; 300-750 MHz) and the Murchison Widefield Array ($\sim$170-200 MHz). The low-frequency data reveal a previously unreported feature in the average profile (at 185 MHz) after accounting for the effects of temporal broadening arising from multi-path scattering due to the Interstellar Medium (ISM). We advance a new method for flux density calibration of beamformed data from the uGMRT and use it to measure the single pulse flux densities across the uGMRT band. Combined with previously published measurements, these flux densities are best fit with a power-law spectrum with a low-frequency turnover. We also use calibrated flux densities to explore the relationship between pulse-to-pulse variability and the spectral index of individual pulses. Our analysis reveals a large scatter in the single-pulse spectral indices and a general tendency for brighter pulses to show a steepening of the spectral index. We also examine the frequency-dependence of the pulse-fluence distribution and its relation to the Stochastic Growth Theory.

==> table2.tex <==
\begin{table*}
\centering
\caption{Log-normal fit parameters of pulse energy distribution for uGMRT Epoch 1 observations.}
\label{tab:fit_e1}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
         & 317 MHz & 350 MHz & 383 MHz & 417 MHz & 450 MHz & 483 MHz & 575 MHz & 625 MHz & 675 MHz & 725 MHz \\ \hline
$\mu$    & 7.87    & 7.60    & 8.02    & 6.74    & 6.62    & -       & 5.94    & 5.97    & 6.16    & 5.70    \\ 
$\sigma$ & -0.58   & 0.56    & -0.50   & -0.51   & 0.54    & -       & 0.39   & 0.41    & 0.43   & 0.45    \\ 
GoF      & 2.12    & 2.72    & 0.45    & 1.32    & 0.88    & -       & 0.30    & 0.65    & 0.78    & 1.01    \\ \hline
\end{tabular}
\end{table*}

\begin{table*}
\centering
\caption{Log-normal fit parameters of pulse energy distribution for uGMRT Epoch 1 observations.}
\label{tab:fit_e2}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
         & 317 MHz & 350 MHz & 383 MHz & 417 MHz & 450 MHz & 483 MHz & 575 MHz & 625 MHz & 675 MHz & 725 MHz \\ \hline
$\mu$    & 7.40    & 7.67    & -       & 6.38    & 6.12    & -       & 5.44    & 5.09    & 5.75    & 5.75    \\ 
$\sigma$ & 0.46    & 0.47    & -       & 0.48    & 0.44    & -       & -0.36   & 0.37    & 0.39    & -0.40   \\ 
GoF      & 0.98    & 0.90    & -       & 0.95    & 0.46    & -       & 0.27    & 0.63    & 0.71    & 0.36    \\ \hline
\end{tabular}
\end{table*}

\begin{comment}
\begin{table*}
\centering
\caption{Log-normal fit parameters of pulse energy distribution for uGMRT Epoch 1 observations.}
\label{tab:fit_e2}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
         & 317 MHz & 350 MHz & 383 MHz & 417 MHz & 450 MHz & 483 MHz & 575 MHz & 625 MHz & 675 MHz & 725 MHz \\ \hline
$\mu$    & 2.76    & 2.98    & -       & 2.75    & 2.27    & -       & 0.04    & 0.61    & 2.31    & 1.80    \\ 
$\sigma$ & 0.46    & 0.47    & -       & 0.48    & 0.44    & -       & -0.36   & 0.37    & 0.39    & -0.40   \\ 
GoF      & 0.98    & 0.90    & -       & 0.95    & 0.46    & -       & 0.27    & 0.63    & 0.71    & 0.36    \\ \hline
\end{tabular}
\end{table*}
\end{comment}

